A Privacy-Aware Bayesian Approach for Combining Classifier and Cluster Ensembles

This paper introduces a privacy-aware Bayesian approach that combines ensembles of classifiers and clusterers to perform semi-supervised and transductive learning. We consider scenarios where instances and their classification/clustering results are distributed across different data sites and have sharing restrictions. As a special case, the privacy aware computation of the model when instances of the target data are distributed across different data sites, is also discussed. Experimental results show that the proposed approach can provide good classification accuracies while adhering to the data/model sharing constraints.

==> algorithm_BC3E.tex <==
\begin{algorithm}[ht]
\caption{--- \textbf{BC\textsuperscript{3}E}}
\label{algo:LearnBC3E}
\begin{footnotesize}
\begin{algorithmic}
\STATE \hspace*{-2mm} {\bf Input:} $\vect{X}$
\STATE \hspace*{-2mm} {\bf Output:} $\vect{\zeta}_{0}$
\STATE {\bf Step 0:} Initialize $\vect{\zeta}_{0}$.
\STATE Until Convergence
\STATE \hspace*{1mm} {\bf Step 1: E-Step}
\STATE \hspace*{2mm} {\bf Step 1a:} Initialize $\{\vect{\zeta}_{n}\}_{n=1}^{N}$.
\STATE \hspace*{3mm} Until Convergence
\STATE \hspace*{3mm} $\forall\text{ }n\in\{1,2,\cdots,N\}$
\STATE \hspace*{4mm} {\bf Step 1b:} Update $\phi_{nmi}$ using Eq.~\eqref{updatephi} $\forall m,i$.
\STATE \hspace*{4mm} Normalize $\vect{\phi}_{nm}$ to 1 $\forall m$.
\STATE \hspace*{4mm} {\bf Step 1c:} Update $\gamma_{ni}$ using Eq.~\eqref{updategamman} $\forall i$.
\STATE \hspace*{1mm} {\bf Step 2: M-Step}
\STATE \hspace*{2mm} {\bf Step 2a:} Update $\beta_{mij}$ using Eq.~\eqref{updatebeta} 
$\forall m,i,j$.
\STATE \hspace*{2mm} Normalize $\vect{\beta}_{mi}$ to 1 $\forall m,i$.
\STATE \hspace*{2mm} {\bf Step 2b:} Maximize~\eqref{updatealpha} w.r.t. $\vect{\alpha}$ with the constraint 
$\vect{\alpha}\ge \vect{0}$. 
\end{algorithmic}
\end{footnotesize}
\end{algorithm}




